Deep Structured Learning for Facial Action Unit Intensity Estimation

We consider the task of automated estimation of facial expression intensity. This involves estimation of multiple output variables (facial action units --- AUs) that are structurally dependent. Their structure arises from statistically induced co-occurrence patterns of AU intensity levels. Modeling this structure is critical for improving the estimation performance; however, this performance is bounded by the quality of the input features extracted from face images. The goal of this paper is to model these structures and estimate complex feature representations simultaneously by combining conditional random field (CRF) encoded AU dependencies with deep learning. To this end, we propose a novel Copula CNN deep learning approach for modeling multivariate ordinal variables. Our model accounts for $ordinal$ structure in output variables and their $non$-$linear$ dependencies via copula functions modeled as cliques of a CRF. These are jointly optimized with deep CNN feature encoding layers using a newly introduced balanced batch iterative training algorithm. We demonstrate the effectiveness of our approach on the task of AU intensity estimation on two benchmark datasets. We show that joint learning of the deep features and the target output structure results in significant performance gains compared to existing deep structured models for analysis of facial expressions.

==> Makefile <==
PROJECT=main

bibtex=bibtex
pdflatex=pdflatex
BIBTEX=$(bibtex) main.aux
BUILDTEX=$(pdflatex) \
		 -halt-on-error \
		--output-directory ./\
		-aux-directory=./\
		-file-line-error \
		$(PROJECT).tex 


all:
	$(BUILDTEX)
	bibtex ${PROJECT}.aux
	$(BUILDTEX)
	$(BUILDTEX)

clean:
	rm -rf build/*


==> misc/alg_2.tex <==
\begin{algorithm}
\textbf{Input:} 
Training data: $\mathcal{D}=\{ {\vec{x}_{i},\vec{y}_{i}}\}_{i=1}^{N}$\\
\hspace{0.95cm} Model parameters: $\Omega=\{W,H,a,b,\sigma\}$\\ 
\hspace{1cm} BBox parameters: $\{B_0,B_1,B_l\}$\\ 
\textbf{Algorithm:} \\
\For{$q \in Q$}{
	\textit{\textit{\# cut out high resolution image}}\\
	$x_{in}^{q}=cutout(x,B_0^q,B_1^q,B_l^q)$\\
	\textit{\textit{\# Train expert model}}\\
	$\Omega^{*}=\mathop {\arg\!\min}\limits_{\Omega_q}E_{r}(x_{in}^{q},y^{q},\Omega)$ \hfill (eq. \ref{eq:cross-entropy-r-ocnn})\\
}
\textbf{Output:} Model parameters: $\Omega*$
\vspace{0.3cm}
\caption{EXO-OCNN learning}
\label{alg2}
\end{algorithm}


==> sec/Makefile <==
PROJECT=main

bibtex=bibtex
pdflatex=pdflatex
BIBTEX=$(bibtex) build/main.aux
BUILDTEX=$(pdflatex) \
		 -halt-on-error \
		--output-directory build \
		-aux-directory=build \
		-file-line-error \
		$(PROJECT).tex 


all:
	$(BUILDTEX)
	bibtex build/${PROJECT}.aux
	$(BUILDTEX)
	$(BUILDTEX)

clean:
	rm -rf build/*


==> tab/cv_table.tex <==
\begin{table}[htbp]
\captionsetup{font=scriptsize}
  \label{tab:cv_exp}%
\small
  \centering
  \caption{\hl{Should this be in supplement?} Performance in terms of ICC of the \ccnn model with different network architectures. We performed a number of experiments in order to find the best architecture for the target problem. The output size of the fcl corresponds to the feature dimension of the facial feature vector $f_d(\vect{x}$. We also applied random cropping with a different windows size where we cut out between $80\%$ and $90\%$ of the original image. The $\lambda$ parameter corresponds to the weight on the L2 regularization. This parameter has to be chosen carefully.  In contrast, the number of CNN-layers and the filter size in each layer result in less significant performance vairations.}
        \begin{tabularx}{\linewidth}{l|XXX|XXX}
    \hline
                                      & \multicolumn{3}{c}{DISFA} & \multicolumn{3}{|c|}{FERA} \\
    \hline
                \textit{fcl size}     & 64                        & \textbf{128}              & 512            & 64   & \textbf{128}  & \textbf{512}   \\
            ICC                       & 0.39                      & \textbf{0.43}             & 0.41           & 0.51 & \textbf{0.63} & \textbf{0.63}  \\
    \hline
    %& & & & & & \\
                \textit{rand. crop}   & 0.8                       & \textbf{0.85}             & 0.9            & 0.8  & \textbf{0.85} & 0.9            \\
            ICC                       & 0.39                      & \textbf{0.43}             & 0.42           & 0.57 & \textbf{0.63} & 0.6            \\
    \hline
            $\lambda$                 & off                       & const.                    & \textbf{tuned} & off  & const.        & \textbf{tuned} \\
            ICC                       & 0.37                      & 0.39                      & \textbf{0.43}  & 0.55 & 0.59          & \textbf{0.63}  \\
    \hline
                \textit{filter size}  & 7                         & \textbf{9}                & 11             & 7    & 9             & \textbf{11}    \\
                ICC                   & 0.41                      & \textbf{0.43}             & 0.42           & 0.61 & 0.63          & \textbf{0.64}  \\
    \hline
                \# \textit{cnn layer} & 2                         & \textbf{3}                & 4              & 2    & \textbf{3}    & 4              \\
            ICC                       & 0.41                      & \textbf{0.43}             & 0.38           & 0.62 & \textbf{0.63} & 0.61           \\
    \hline
    \end{tabularx}%
\end{table}%



==> tab/disfa_partially.tex <==
% Table generated by Excel2LaTeX from sheet 'disfa_partially'
\begin{table}[htbp]
\captionsetup{font=scriptsize}
  \footnotesize
  \centering
\caption{The intensity estimation results (ICC) on the DISFA testset, trained on the training sets from all three databases. We compare \scnnC, the structured models with linear potentials with \ccnn-IT(*), the model that uses copula potentials. The AUs that are highlighted with the Asterix were removed from the training set.}
\begin{tabularx}{\linewidth}{c|XXXXXXXXXXXX}
\hline
AU:           & 1            & 2            & 4            & 5            & 6            & 9            & 12            & 15           & 17           & 20           & 25           & 26            \\
\hline
        \ccnn & .17          & \textbf{.14} & \textbf{.60} & .07          & \textbf{.65} & \textbf{.54} & $.63^{\ast}$  & \textbf{.43} & .36          & \textbf{.28} & \textbf{.76} & \textbf{.53 } \\
        \scnn & .15          & .12          & .43          & .06          & .61          & .53          & $.51^{\ast}$  & \textbf{.43} & .37          & \textbf{.28} & \textbf{.76} & .52           \\
\hline
        \ccnn & .14          & .11          & .42          & .06          & $.22^{\ast}$          & \textbf{.53} & $.41^{\ast}$  & .42          & .36          & .27          & \textbf{.76} & .52           \\
        \scnn & .04          & .05          & .31          & .01          & $.21^{\ast}$          & .39          & $.42^{\ast}$  & .29          & .19          & .03          & .64          & .34           \\
\hline
        \ccnn & \textbf{.20} & .12          & .46          & \textbf{.08} & .48          & .44          & \textbf{.73 } & .29          & \textbf{.45} & .21          & .60          & .46           \\
        \scnn & \textbf{.20} & .07          & .46          & \textbf{.08} & .48          & .41          & \textbf{.73 } & .29          & .41          & .21          & .60          & .44           \\
\hline
        \ccnn         & --           & --           & $.23^{\ast}$          & --           & $.22^{\ast}$          & $.21^{\ast}$          & $.38^{\ast}$           & --           & $.21^{\ast}$          & $.13^{\ast}$          & $.51^{\ast}$          & $.24^{\ast}$           \\
        \scnn         & --           & --           & $.18^{\ast}$          & --           & $.20^{\ast}$          & $.14^{\ast}$          & $.37^{\ast}$           & --           & $.19^{\ast}$          & $.11^{\ast}$          & $.41^{\ast}$          & $.22^{\ast}$           \\
\hline
\end{tabularx}%
\label{tab:addlabel}%
\end{table}%
